Low Cost, Open-Source Testbed to Enable Full-Sized Automated Vehicle Research

An open-source vehicle testbed to enable the exploration of automation technologies for road vehicles is presented. The platform hardware and software, based on the Robot Operating System (ROS), are detailed. Two methods are discussed for enabling the remote control of a vehicle (in this case, an electric 2013 Ford Focus). The first approach used digital filtering of Controller Area Network (CAN) messages. In the case of the test vehicle, this approach allowed for the control of acceleration from a tap-point on the CAN bus and the OBD-II port. The second approach, based on the emulation of the analog output(s) of a vehicle's accelerator pedal, brake pedal, and steering torque sensors, is more generally applicable and, in the test vehicle, allowed for the full control vehicle acceleration, braking, and steering. To demonstrate the utility of the testbed for vehicle automation research, system identification was performed on the test vehicle and speed and steering controllers were designed to allow the vehicle to follow a predetermined path. The resulting system was shown to be differentially flat, and a high level path following algorithm was developed using the differentially flat properties and state feedback. The path following algorithm is experimentally validated on the automation testbed developed in the paper.

==> abstract.tex <==
% As a general rule, do not put math, special symbols or citations
% in the abstract
\begin{abstract}
An open-source vehicle automation methodology and platform for road vehicles (cars and trucks) is presented. The platform hardware and software, based on the Robot Operating System (ROS), are detailed. Two strategies are discussed for enabling the remote control of a vehicle (in this case, an electric 2013 Ford Focus). The first approach used digital filtering of Controller Area Network (CAN) messages.  In the case of the test vehicle, this approach allowed for the control of acceleration from a tap-point on the CAN bus and the OBD-II port. The second approach, based on the emulation of the analog output(s) of a vehicle's accelerator pedal, brake pedal, and steering torque sensors, is more generally applicable and, in the test vehicle, allowed for the full control vehicle acceleration, braking, and steering.  To demonstrate the utility of the methodology and platform for vehicle automation research, system identification was performed on the test vehicle and speed and steering controllers were designed to allow the vehicle to follow a pre-determined path. The resulting system was shown to be differentially flat, and a high level path following algorithm was developed using the differentially flat properties and state feedback. Experimental results are presented.


%An open-source automation platform for full-sized automobiles is presented. Two strategies are discussed for enabling remote control of a 2013 Ford Focus EV. The first approach uses digital filtering of CAN messages to control vehicle acceleration. This approach was used to control acceleration from a tap-point on the CAN bus, and through the OBD-II port. The second approach emulates sensor outputs from the vehicles accelerator pedal, brake pedal, and steering torque sensors to control the acceleration, braking, and steering. System identification is performed to obtain a vehicle model and design controllers. The system is shown to be differentially flat, and a high level path following algorithm is developed using the differentially flat properties and state feedback. The platform hardware and software are detailed and experimental results of full-sized vehicle automation are presented. The platform is designed using the Robot Operating System (ROS).

%First, digital control messages are filtered and manipulated on the CAN bus to cause vehicle acceleration. The CAN messages are filtered at a tap-point on the bus, and through the OBD-II port. Second, sensor input to CAN modules is emulated by a microcontroller to dictate vehicle behavior. System identification is performed to obtain a vehicle model and design controllers. The system is shown to be differentially flat, and a high level path following algorithm is developed using the differentially flat properties and state feedback. The platform hardware and software are detailed and experimental results of full-sized vehicle automation are presented. The platform is designed using the Robot Operating System (ROS).

\end{abstract}

